Data Analytics Driven Controlling: bridging statistical modeling and managerial intuition

Strategic planning in a corporate environment is often based on experience and intuition, although internal data is usually available and can be a valuable source of information. Predicting merger & acquisition (M&A) events is at the heart of strategic management, yet not sufficiently motivated by data analytics driven controlling. One of the main obstacles in using e.g. count data time series for M&A seems to be the fact that the intensity of M&A is time varying at least in certain business sectors, e.g. communications. We propose a new automatic procedure to bridge this obstacle using novel statistical methods. The proposed approach allows for a selection of adaptive windows in count data sets by detecting significant changes in the intensity of events. We test the efficacy of the proposed method on a simulated count data set and put it into action on various M&A data sets. It is robust to aberrant behaviour and generates accurate forecasts for the evaluated business sectors. It also provides guidance for an a-priori selection of fixed windows for forecasting. Furthermore, it can be generalized to other business lines, e.g. for managing supply chains, sales forecasts, or call center arrivals, thus giving managers new ways for incorporating statistical modeling in strategic planning decisions.

==> backup.tex <==
\cite{noauthor_mergers_2012} {\color{red} (fix this reference)}  outlines that the process of M\&As happens in 10 phases and requires a significant amount of preparation. While these events should not be considered to occur randomly from the perspective of an insider, information on their announcement is held back from the public in most of these stages, such that researchers can treat them as, to a certain extent, randomly occurring events created by some explanatory factors that can be derived from economic theory. \cite{rhodeskropf_market_2004} find that market misvaluation drives merger activity. Empirical evidence strongly suggests that mergers are often clustered in time, a phenomenon that is still not fully explainable \citep{maksimovic_private_2013}.

\cite{ahern_importance_2014} find that M\&A activity is subject to network effects and that these waves largely occur within industries, but can also be transmitted to connected industries. \cite{harford_what_2005} studies the drivers of such merger waves and attributes them to economic, regulatory and technological shocks. \cite{martynova_century_2005} study several merger waves since the end of the 19th century. They confirm that waves are preceded by shocks and driven by market misvaluation, but conclude that these waves are diverse in structure and patterns.

\cite{zhao_technological_2009} evaluates the correlation between technological innovation and merger activity and finds that it affects firms' acquisition decisions, and these activities subsequently benefit their innovation efforts. This indicates that especially innovative sectors, such as technology or financials can be expected to have a high degree of M\&A activity. \cite{cai_anticipation_2011} examine anticipation effects and find that the announcement of a M\&A in a market does not necessarily lead to further bids, and that increased bidding activity among competitors often precedes merger waves. \cite{netter_implications_2011} study a dataset that also includes small and private M\&As and conclude that wave-like patterns largely disappear through including them, but they find evidence for seasonality in their announcement date. 

We conclude that data on M\&As should be evaluated per industry. In addition, while international industry-specific and cross-industry networks can be assumed, a geographic separation due to differences in regulation, innovation power, technology, and stock markets seems feasible. Furthermore, shocks of any kind, even if they lead to merger waves, are difficult to predict. Wave patterns seem to be heterogeneous and differ both in time and in industries. Given the complex structure of the underlying data, a predictive model could be identified through aggregating the acquired knowledge and tailored to specific industries and markets. Alternatively, a generic time-series model could be applied. While a co-variate based model provides explainability to the user, it requires manual efforts to gather data and incorporate expert knowledge to define relevant variables and calibrate their impact on a predictive model. However, data gathering can be time-consuming and expensive, and knowledge about modeling heterogeneous industries in a specific application requires domain knowledge, that is often scarce and narrowed to said application. Therefore, generic time series models are an attractive alternative, as they can be adapted to any other dataset with comparable structure. However, such models need to be robust to non-stationarity, seasonality, and wave patterns that limit the predictive power of common models like those of the autoregressive family.

In addition, the length of homogenous parameter time windows is in absence of sophisticated methods often chosen arbitrarily, but forecasting performance differs with window size \cite{inoue_rolling_2017}.
As a real world example, \ref{fig:movingaverages} shows the frequency of mergers \& acquisitions (M\&A) in the German energy market. Clearly, the observed frequency is time-varying, and a forecast generated from the whole dataset would be inaccurate, see e.g. \citep{spokoiny_multiscale_2009} who address this problem by introducing a local change point analysis approach. This approach is part of a branch of literature focusing on change point detection (CPD), which focuses on testing procedures to identify structural breaks in time series.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.90\textwidth]{images/Movingaverages.png}
    \caption{{\color{sapphirecrayola} Time series of number of mergers and acquisitions}, with moving average curve of {\color{orange} 1 year} and {\color{aoenglish}3 year}}
    \label{fig:movingaverages}
\end{figure}
\sloppy
CPD literature has been widely divided into probabilistic and non-probabilistic methods. 
A summary can be viewed in \cite{aminikhanghahi_survey_2017}, \cite{chen_parametric_2011}, and \cite{eckley_analysis_2011}. 
Many methodologies discussed by the researchers working in the field are limited to single CPD.
The literature on multiple is mainly focused on likelihood ratio (LR) tests and Bayesian tests. 
The two approaches have been evaluated as the most effective for CPD and are therefore amongst the first few choices for determining the homogeneous time intervals. 

Naturally, the algorithms for multiple CPD are computationally expensive because they have to locate change points in a large pool of possible positions in a time series. Bayesian methods with computational cost of $\mathcal{O}(n)$ are faster than likelihood based approach in general \citep{aminikhanghahi_survey_2017}. However, Bayesian methods require apriori information concerning the position and number of change points which is not generally available in practice. Alternatively, definition of prior on length of the segments in which the time series is divided should be specified. While there are common choices available for the priors such as geometric distribution, the estimation of parameters of the posteriors by sampling (or approximating) through methods like MCMC are computationally intensive. Furthermore, it is noted that the choice of prior and the parameter space affects the test results for the CPD. In many cases, wrong assumptions on the prior may lead to the selection of simple models (with no change points), hence generating biased results \citep{eckley_analysis_2011}. 

Likelihood based approaches have an advantage over Bayesian because they do not require any apriori information.
However, they can be computationally challenging.
They have been extended to detect changes in mean related to various continuous distributions including normal \citep{chen_change_1999}, gamma \citep{hsu_detecting_1979}, and exponential \citep{haccou_likelihood_1987}. 
The detection of change of mean in discrete probability models, however, has seen very little contribution. While CPD in binomial probability model have been considered both through likelihood perspective, for example by \cite{hinkley_inference_1970} and Bayesian point of view, for example by \cite{smith_bayesian_1975}, the mean change detection in Poisson probability model has only been evaluated through Bayesian approach like in \cite{yang_bayesian_2001} and not from a likelihood perspective.
\cite{chen_parametric_2011} provides the null distribution of LR test for Poisson distributed random variables, but they do not evaluate the efficacy of procedure on real life data. 

Inspired by the growing practical appearance of discrete data, e.g. M\&A in figure \ref{fig:movingaverages} with small sample size and small mean, we extend the likelihood based approach to the Poisson distribution which is a natural choice to model such data. 
Specifically, the issue of choice of window length where the mean can be assumed constant (interval of homogeneity) has to be addressed: small windows lead to high variability of the estimators, large windows increases the delay and the location error in change-point detection \citep{hardle_local_2015} (see figure \ref{fig:movingaverages}). The general framework for selection of these intervals of homogeneity was first introduced by \cite{spokoiny_estimation_1998} as local parametric approach (LPA). Later, LPA was adapted for different models such as multiplicative error models in \cite{hardle_adaptive_2014} and \cite{hardle_local_2015}. Very recently, \cite{klochkov_localizing_2019} localized multivariate CaViar model using the same methodology. They also combine LPA with Multiplier Bootstrap (MBS) which inherently deals with issues of small sample size and model misspecification \citep{spokoiny_bootstrap_2015} and yields the critical values for the solution of the homogeneous intervals.


\begin{enumerate}
\item\textbf{Initialization}: Select \(I_0, I_1, I_2,\) and define \(J_1=I_1\backslash I_0, (\forall \tau \in J_1),\)  \(A_{1,\tau}=[i_0-n_2, \tau] \), \(B_{1,\tau}=(\tau, i_0] \).
\item\textbf{Iteration}: For each iteration, select \(I_{k-1}, I_k, I_{k+1},\), 
\(J_k=I_k\backslash I_{k-1},(\forall \tau \in J_k)\) 
\(A_{k,\tau}=[i_0-n_{k+1}, \tau],\) \(B_{k,\tau}=(\tau, i_0] \).
\item\textbf{Testing homogeneity}:
Calculate test statistics in equation (\ref{eq:T}) and select critical value with multiplier bootstrap. Test hypothesis in equation (\ref{eq:hypothesis}) using equation (\ref{eq:maxT}).  
\item\textbf{Loop}: If \(I_k\) is accepted, take the next interval \(I_{k+1}\). Otherwise set \(\widehat{I}\) to the latest non rejected \(I_k\). 
\item\textbf{Adaptive estimator}:  Take  interval \(\widehat{I}\) as interval of homogeneity and \(\widehat{\theta}_{i_0} = \widehat{\theta}_{\widehat{I}} \) as adaptive estimate of \(\widehat{I}\).
Repeat the procedure for each point in time (different \(i_0\))
\end{enumerate}
